Masses of a Fourth Generation with Two Higgs Doublets

We use sampling techniques to find robust constraints on the masses of a possible fourth sequential fermion generation from electroweak oblique variables. We find that in the case of a light (115 GeV) Higgs from a single electroweak symmetry breaking doublet, inverted mass hierarchies are possible for both quarks and leptons, but a mass splitting more than M(W) in the quark sector is unlikely. We also find constraints in the case of a heavy (600 GeV) Higgs in a single doublet model. As recent data from the Large Hadron Collider hints at the existence of a resonance at 124.5 GeV and a single Higgs doublet at that mass is inconsistent with a fourth fermion generation, we examine a type II two Higgs doublet model. In this model, there are ranges of parameter space where the Higgs sector can potentially counteract the effects of the fourth generation. Even so, we find that such scenarios produce qualitatively similar fermion mass distributions.

==> CHANGES <==
Modifications from version submitted to PRD.

1) Replaced \date{\today} with \date{20 June 2012}

2) New text starting on pg 7 left hand side just after citation 45, including
citation of Chen & He, arXiv:1202.3072; then more on the right hand side where
Equation 3 once was.

3) "4G Standard Model" replaced with "4G scenario" in 2 places on 1st page..
We should use "Standard Model" to be 3G, 1 Higgs doublet only.

4) Dropped reference to HiggsBounds from acknowledgements, as we do not use it.

5) Uniformly used $m(thing)$ rather than $M_{thing}$ or $m_{thing}, except for
thing = W.

6) Included over/underflow bins in calculating the normalization.

7) Added a sentence of explanation at the reference to Figure 1 to try to
explain it better.

8) Took a go at Zbb and other possible constraints in top left of page 7.
